Adjusting for Autocorrelated Errors in Neural Networks for Time Series

An increasing body of research focuses on using neural networks to model time series. A common assumption in training neural networks via maximum likelihood estimation on time series is that the errors across time steps are uncorrelated. However, errors are actually autocorrelated in many cases due to the temporality of the data, which makes such maximum likelihood estimations inaccurate. In this paper, in order to adjust for autocorrelated errors, we propose to learn the autocorrelation coefficient jointly with the model parameters. In our experiments, we verify the effectiveness of our approach on time series forecasting. Results across a wide range of real-world datasets with various state-of-the-art models show that our method enhances performance in almost all cases. Based on these results, we suggest empirical critical values to determine the severity of autocorrelated errors. We also analyze several aspects of our method to demonstrate its advantages. Finally, other time series tasks are also considered to validate that our method is not restricted to only forecasting.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}[leftmargin=20pt]

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
  \answerYes{Summarized in last paragraph in the Section~\ref{sec:intro}.}
  \item Did you describe the limitations of your work?
  \answerYes{See Section~\ref{ssec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
  \answerYes{See Section~\ref{sec:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
  \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
  \answerYes{The (anonymized) URL is in the second to last paragraph in Section~\ref{sec:intro}. We also submit the code in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{ssec:models}, Section~\ref{ssec:datasets}, Section~\ref{ssec:all_results}, and Appendix~\ref{app:all_hyper}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All experiments are run multiple times. Error bars are reported in the form of t-tests.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{Experiments do not require high-end GPUs.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  \answerYes{We used existing datasets and we cite them in Section~\ref{ssec:datasets} and Appendix~\ref{app:detail_data}.}
  \item Did you mention the license of the assets?
  \answerNo{We were unable to find the license for the datasets, but we do cite the original papers and the URLs.}
  \item Did you include any new assets either in the supplemental material or as a URL?
  \answerYes{The new asset is my code. The (anonymized) URL is in the second to last paragraph in the Section~\ref{sec:intro} and the code is in the supplementary material }
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  \answerNo{We are unable to find the information.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  \answerNo{Our data are either anonymized or do not tied to an individual (For example, traffic data is aggregated over all cars on roads).} 
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
  \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA{}
\end{enumerate}

\end{enumerate}

==> figures/sizes.tex <==
\begin{figure}[t!]

\centering
\includegraphics[width=0.55\columnwidth]{images/sizes.pdf}

\caption{Results of training \textsf{LSTM} on the \texttt{Traffic} dataset with different numbers of layers and hidden units averaged over $30$ runs using both the w/o and w/ methods. In the upper right subfigure, $y$-axis is the relative improvement of using w/ over w/o.}
\label{fig:sizes}

\end{figure}
